Encoding word order in complex embeddings

Sequential word order is important when processing text. Currently, neural networks (NNs) address this by modeling word position using position embeddings. The problem is that position embeddings capture the position of individual words, but not the ordered relationship (e.g., adjacency or precedence) between individual word positions. We present a novel and principled solution for modeling both the global absolute positions of words and their order relationships. Our solution generalizes word embeddings, previously defined as independent vectors, to continuous word functions over a variable (position). The benefit of continuous functions over variable positions is that word representations shift smoothly with increasing positions. Hence, word representations in different positions can correlate with each other in a continuous function. The general solution of these functions is extended to complex-valued domain due to richer representations. We extend CNN, RNN and Transformer NNs to complex-valued versions to incorporate our complex embedding (we make all code available). Experiments on text classification, machine translation and language modeling show gains over both classical word embeddings and position-enriched word embeddings. To our knowledge, this is the first work in NLP to link imaginary numbers in complex-valued representations to concrete meanings (i.e., word order).

==> case_study.tex <==
\subsection{Case Studies}
\label{se:5-4}

\begin{figure*}[htbp] 
\centering 
\includegraphics[height=5cm, width=15cm]{figures/semantic_simliarity.pdf}
\caption{Distances of sliding n-grams in different sentences using trained embedding in real-valued Word2vec (a), \textbf{TPE-reduce} \cite{vaswani2017attention} (b), and \textbf{Complex-order} (c) respectively. Yellow-colored indicates that similarity is highest. The word order of the bold part has changed.} 
\label{fig:semantic_simliarity}
\vspace{-10px}
\end{figure*}

% \begin{table}[ht]
% \centering 
% \begin{tabular}{ccc}
% \toprule[1pt]
% Layer Type & Complexity & Sequential\\
% ~&per Layer& Operations\\
% \midrule[0.5pt]
% CNN & $\mathcal{O}(knd^2)$ & $\mathcal{O}(1)$ \\
% CNN-PT/TPE-concat & $\mathcal{O}(2knd^2)$ & $\mathcal{O}(1)$ \\
% CNN-complex-order & $\mathcal{O}(knd^2)$ & $\mathcal{O}(1)$ \\
% % BiLSTM & $\mathcal{O}(nd^2)$ & $\mathcal{O}(n)$ \\
% % BiLSTM-p-complex & $\mathcal{O}(nd^2)$ & $\mathcal{O}(n)$ \\
% \bottomrule[1pt]
% \end{tabular}
% \caption{Per-layer complexity and minimal sequential operations for different layer types. n is the sequence length, d is the embedding dimension, k is the kernel size of convolutions.}
% % $n$ is the sequence length, $d_{model}$ is the representation dimension and $R$ is the rank in the tensor representation.
% \label{Tabel:comp}
% \end{table}


% the first is the experimental effect, the complex-embedding performs better than position encoding methods on MR and SUBJ \ref{3-2}.

In order to understand the difference between our propose complex-valued word embedding and previous embedding approaches e.g. vanilla word embedding \cite{mikolov2013efficient} and the combine embedding between word embedding and position embedding which is calculated in Eq. \ref{eq:position_embedding} \cite{vaswani2017attention}, we select a document pair and calculate the similarity scores between all the sliding $N$-gram based the fine-tuned embedding after training. The similarity scores are based on the cosine similarity for both real-valued and complex-valued vectors.

In the Fig. \ref{fig:semantic_simliarity} (a, b, c),
%  We selected two cases from the MR dataset, position influence sentence semantics and position do not affect sentence semantics, respectively. Real-valued embedding and complex-embedding are trained by CNN-complex-order on MR, position embedding is calculated according to Eq. \ref{eq:position_embedding}, the representation of n-grams is derived from the accumulation of word embeddings. 
%  Fig. \ref{fig:semantic_simliarity} provides cosine similarity between different n-grams for different embeddings on sentences. 
`except good' and `good except' are the significant signals which are related to the final label i.e. negative or positive, but with a different order between `except' and `good'. The vanilla Word2vec vector in Fig. \ref{fig:semantic_simliarity} a without position embedding fails to capture their difference and tends to predict that the two tri-grams have similar representations. While our propose word embedding in Fig. \ref{fig:semantic_simliarity} c can be sensitive to the positions. However, the semantic representations in  Fig. \ref{fig:semantic_simliarity} b with sum between word embedding and position embedding \cite{vaswani2017attention} is largely biased by the absolute position embeddings, lead to sensitivity of position but lacking modelling semantic aspect; therefore it may highly rely on large-scale training data to fine-tune and relief the effect of noisy dimensions in position embedding especially with big variances.
In some sense, the word semantic information and its positional information are decoupled, since the $pos$ varaible which is used to encode the position cannot affect mean value of the functions which is linearly correlated to its semantic part, i.e., amplitude vectors. 

% Instead, our proposed general complex embedding for combining word embedding and position embedding cannot only capture both the absolute positions and relative orders, but also almost preserve the original semantic representation which is trained from large-scale external corpora  due to that the phrase vectors which encode the position cannot affect the amplitude vectors in term of the mean value. 
% Formally, $ \int_{-\pi}^{\pi} re^{i\theta} d\theta =  $



% in \ref{fig:semantic_simliarity}(a,b,c). In Fig. \ref{fig:semantic_simliarity}(a) the representation of 3-grams are based on Real-valued embedding, which not contain word order information and can't distinguish `except good' and `good except'. The two phrases are not the most relevant in Fig. \ref{fig:semantic_simliarity}(b) and Fig. \ref{fig:semantic_simliarity}(c), which can be beneficial to make correct judgments on sentences. However, compare Fig \ref{fig:semantic_simliarity}{b} and Fig \ref{fig:semantic_simliarity}{e}, we can find that the picture has not changed since the sentence was changed, because of the value of position embedding is too large.  

% In the \ref{fig:semantic_simliarity}(d,e,f), `serial killer jeffrey dahmer' become `jeffrey dahmer serial killer' semantics has not benn changed. The 4-grams representation based on Real-valued embedding and complex-embedding is most similar on semantics. However, the diagonal of Fig. \ref{fig:semantic_simliarity}(e) based on Real-valued and position embeddings \cite{vaswani2017attention} are most similar, this proves that Real-valued and position embedding require more parameters to learn the balance between location information and semantic information. Complex-embedding can smooth semantic and word order information without relying on parameters. 

%   By comparing with Fig \ref{fig:semantic_simliarity}, it can be found that the picture has not changed since the sentence was changed.


% sentence 1: `not an objectionable or dull film it merely lacks everything except good intentions' and `everything about the quiet american is good except its timing'.

% sentence 2:`does what should seem impossible it makes serial killer jeffrey dahmer boring' and `chilling but uncommercial look into the mind of jeffrey dahmer serial killer'.



==> old/affine_map.tex <==
Formally, we prove the following claim that there is a unique solution to meet the above two properties under the assumption that the transformation function is limited to be linear since it could be a simplest case.  \benyou{why  discuss  only the linear function?}
\begin{thm}
There exists a unique bounded function $g(\cdot): \mathbb{N} \rightarrow \mathbb{C}$ satisfying properties 1 and properties 2, given by 
\begin{equation}
\label{eq:solution}
    g(pos) = \left( z_3 - \frac{z_2}{1-z_1} \right)  z_1^{pos} + \frac{z_2}{1-z_1}, \vert z_1 \leq 1 \vert
\end{equation}
such that a linear function $f(x)=wx+b$, where $w$ and $b$ are functions parameterized by the offset distance $n$, can convey a position-free relative-distance transformation like
\begin{equation}
\label{eq:condition}
\begin{aligned}
    g(pos+n) &= w(n)g(pos) + b(n) \\
    w^*(n) &= z_1^n \\ 
    b^*(n) &= \frac{1-z_1^n}{1-z_1} z_2  \\ 
\end{aligned}
\end{equation}
where complex constant values $z_1, z_2, z_3 \in \mathbb{C}$ depend solely on $j,d$ which are omitted.
\end{thm}

\jakob{I am having trouble parsing the exact statement of the claim. In particular it's hard to see whether the conditions in (\ref{eq:condition}) are \emph{consequences} of the claim, or whether they are \emph{assumptions} (also, what do the asterisks mean? -- Are they only defined in the full proof in the appendix?)}




\begin{proof} 
For $g(pos+n_1+n_2)$ with $n=n_1+n_2$, by comparing two transformations i.e. $n_1$-transformation and $n_2$-transformation and one transformation i.e.  $(n_1+n_2)$-transformation, we have $w(n_1)w(n_2)g(pos)+ w(n_1) b(n_2) + b(n_1) =  w(n_1+n_2)g(pos) + b(n_1+n_2)$. Since both the coefficient terms and constant terms should be consistent, $w(n_1+n_2) = w(n_1)w(n_2)$ and $b(n_2+n_1) = w(n_1) b(n_2) + b(n_1)$. Finally we can first get solution for $w(\cdot)$ by using  induction in integer domain. Then the solution of $w(\cdot)$ can be inserted in $b(n_2+n_1) = w(n_1) b(n_2) + b(n_1)$ to get the solution for $b(\cdot)$ by using induction in integer domain as well. Noting that both the two solutions are also valid for the real domain $\mathbb{R}$. By assuming the initial value for $w(\cdot)$,  $b(\cdot)$ and  $f(\cdot)$  as any complex numbers $z_1,z_2,z_3$ respectively, the final solution is solved as Eq.~\ref{eq:solution}. For a detailed proof, please refer to Appendix. 


% From $f_{j,k}(Pos+m) = f_{j,k}(((Pos+n)+...)+n), \forall n$, comparing the coefficients on both sides of the equation, we can get $A(Pos,k) = e^{(-\alpha+i\beta)Pos}$ and $B(Pos,k) = \lambda_0 e^{i\theta_0}(1-e^{(-\alpha+i\beta) Pos})$ given the boundedness condition of $A(Pos,k)$ and $B(Pos,k)$, while $i$ is the imaginary unit. Then we insert $A(Pos,k)$ and $B(Pos,k)$ back to Eq.~\ref{eq:solution} and immediately obtain $f_{j,k}(Pos) = \lambda e^{i\theta} e^{(-\alpha+i\beta)Pos} + \lambda_0 e^{i\theta_0}$. For a detailed proof, please refer to Appendix. 
\end{proof} 

\begin{figure}
    \centering
    \includegraphics[width=50mm]{figures/complex-crop.pdf}
    \caption{complex number in Cartesian plane and polar plane.}
    \label{fig:complexnumber}
\end{figure}

\subsection {Deriving to our Complex-valued Word Embedding}

As shown in Eq.~\ref{eq:solution}, there are generally three complex-valued parameter i.e. six real-valued number for each dimension $d$ of representation of word $w_j$, corresponding to the initial values of $g^*(\cdot)$, $w^*(\cdot)$ and $b^*(\cdot)$ respectively.  By this general solution, six parameters needs be trained  to get a $d$-dimension representation for a word.
Since $pos$ is the independent variable in the functions $g^*(\cdot)$, the total parameters for word embedding is not related to $pos$ and it is possible to model long enough sentences.
There are $6\times D \times \vert \mathbb{W} \vert$ parameters with D-dimensional word vectors and $\vert \mathbb{W} \vert$ words, while the previous works \citep{mikolov2013efficient,pennington2014glove} usually have $ D \times \vert \mathbb{W} \vert$ parameters for embedding lookup table. To save parameters from the application point of view, many variants of complex embedding can be chosen to specialize in some specific cases of the general solution. In this section, we will give two main effective variants.

First, in this work, we can specifically set $z_2$ as zero, i.e., it removes the constant terms in the  linear transformation without harming the Position-free relative-distance transformation. To recap, $z= re^{i\theta}$ in exponential form can be transformed in Cartesian plane as a standard form with real and imaginary parts, i.e., $z= re^{i\theta} = r(\cos \theta + i\sin \theta)$ , where r and $\theta$ are the \textit{modulus} ($\vert z_1 \vert = r_1$) and \textit{argument} respectively,  as shown in Fig~\ref{fig:complexnumber}.  The general solution of $g(\cdot)$ degenerates to $g(pos) =  z_3 z_1^{pos}$ in the case $z_2 = 0$.  $g(\cdot)$ can be written as 

\begin{equation}
\label{eq:g_new}
\begin{aligned}
    g(pos) &=z_3 z_1^{pos} = r_3e^{i\theta_3} (r_1e^{i\theta_1})^{pos} \\
           &=r_3 r_1^{pos} e^{i(\theta_3+\theta_1 pos)}  \\
           & constrained ~ by~  \vert r_1 \vert \leq 1
\end{aligned}
\end{equation}

With setting $r_1 = 1$, we can avoid to optimize a objective with constrains. Now it can be a optimization problem without any constrains, under the definition $g(pos) = r_3 e^{i(\theta_3+\theta_1 pos)}$. To make it clearer, we replace the variable $r_3$ with general $r$, $\theta_3$ with gernal $\theta$, and $\theta_1$ with $2pi \omega$,
\begin{equation}
    g(pos) = r e^{i(\theta+  \omega  pos)}.
\end{equation} 
 $r$ is the amplitude term, $\theta$ is the initial phase term and $ \frac{ \omega}{2\pi}$ is the frequency (the period term is its reciprocal $\frac{2\pi}{\omega}$). In order to save parameters, $\theta$ is also setted as 0. In our work, the final function is defined as $g(\cdot)=r e^{ i \omega  pos} $ parameterized by $r$ and $\omega$， leading to $ 2 D \times \vert \mathbb{W} \vert$ in total. 





% complex number is composed of a real part and imagery part like $z = a+bi$ in , where $i$ is the square root of $-1$, i.e., $i=\sqrt{-1}$. $z$ can be rewritten as 


% Based on Sec. \ref{sec:encoding_relative_position}, complex-valued function with formulation $f_{j,k}(Pos) = \lambda e^{i\theta} e^{(-\alpha+i\beta)Pos}$ is a natural solution to meet the above properties. 
% %The claim above allows us to represent the $j$-th word $w_j$ at position $Pos$ as $\bm{f(j,Pos)} = [\lambda_{j,1}e^{i\theta_{j,1}}e^{(-\alpha_{j,1}+i\beta_{j,1}) Pos},...,\\ \lambda_{j,K}e^{i\theta_{j,K}}e^{(-\alpha_{j,K}+i\beta_{j,K}) Pos}]'$. 
% We first remove the decaying term $-\alpha$, ensuring the amplitudes of position embedding stay constant for all the positions, in the belief that each position should be treated equally. The initial phases $\theta$ and constant terms $\lambda_0 e^{i\theta_0}$ are also set to zeros in our study for simplification purposes, and we will investigate their effect on future work. 
% % Without loss of generality (we will explain it later), 
% Therefore, we choose the following function,
% \begin{equation}~\label{eq:f_solution}
% \bm{f}_{j,k}^{\bm{*}}(Pos) = \lambda_{j,k}e^{i \beta Pos}
% \end{equation}

% The period of function which corresponds to the k-th dimension of word $w_j$ is $p_{j,k} = \frac{2\pi}{\beta_{j,K}}$, while $\lambda_{j,k}$ is the amplitude.

\section{Complex-valued word Embedding}


To model word order utilizing invariant relative-distance transformation, for each word, each dimension of its embedded representation is represented as a continuous function over positions $pos$. In applications, the value of the variable $pos$ is discrete and ranged only in integer domain $\mathbb{N}$. Therefore,  the proposed embedding can be also considered as a map based on two input invariable i.e. word index $j$ and $Pos$. $\mathscr{F}: \mathbb{N} \times \mathbb{N} \rightarrow \mathbb{C}^K $, $\mathbb{C}$ here is the complex-valued field instead of continuous function space. 

% In this paper we generalize the range of the mapping from $ \mathcal{R}^K $ to $ \mathcal{C}^K$. Moreover, we link the word position to the embedding, thus the sequential information can be perceived even in position-unaware neural network structures \footnote{We argue that CNN can only perceive the position of each word in the local context/windows which may not have well-managed borders but not absolute position in a global context.}. As a result, the word embedding is a map $\mathscr{F}: \mathcal{N} \times \mathcal{N} \rightarrow \mathcal{C}^K $ in this work.
